Day-ahead time series forecasting: application to capacity planning

In the context of capacity planning, forecasting the evolution of informatics servers usage enables companies to better manage their computational resources. We address this problem by collecting key indicator time series and propose to forecast their evolution a day-ahead. Our method assumes that data is structured by a daily seasonality, but also that there is typical evolution of indicators within a day. Then, it uses the combination of a clustering algorithm and Markov Models to produce day-ahead forecasts. Our experiments on real datasets show that the data satisfies our assumption and that, in the case study, our method outperforms classical approaches (AR, Holt-Winters).

==> macro-fr.tex <==
\usepackage{soul}
\usepackage[utf8]{inputenc}
\usepackage{verbatim} % underline align
\usepackage[normalem]{ulem} 
%% Macro Thomas
\usepackage{amssymb,amsmath,amsthm}
\usepackage{color}
\usepackage{graphicx}
\usepackage{mathrsfs} % math script letters \mathscr{.}
\usepackage[table,dvipsnames]{xcolor}
\usepackage{vhistory} % versions
\graphicspath{ {images/} }

\makeatletter
\providecommand{\bigsqcap}{%
  \mathop{%
    \mathpalette\@updown\bigsqcup
  }%
}
\newcommand*{\@updown}[2]{%
  \rotatebox[origin=c]{180}{$\m@th#1#2$}%
}
\makeatother

% Page format
\usepackage[left=2cm,right=2cm,top=2cm,bottom=2cm]{geometry}
\usepackage{fancyhdr}
\pagestyle{fancy}
\renewcommand\headrulewidth{1pt}
%\fancyhead[LO]{\it \@title}
%\fancyhead[RO]{\it \title}
%\fancyhead[C]{}
%\fancyhead[RO]{\it \@title}
\fancyhead[LE]{\it \@title - \@author}
\fancyhead[RE]{}
%\fancyfoot[L]{}
\fancyfoot[CO]{}
\fancyfoot[CE]{}
\fancyfoot[LE]{\thepage}
\fancyfoot[RO]{\thepage}

\newtheorem{prop}{Property}
\newtheorem{ex}{Example}
\newtheorem{defdef}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{example}{Example}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}

\newenvironment{wordabout}[1]{\begin{trivlist}\item[]\textbf{#1.}}{\end{trivlist}}
\newenvironment{nonumberedmath}[1]{\begin{trivlist}\item[]\textbf{#1}\it}{\end{trivlist}}
\newenvironment{proofs}[1]{\begin{trivlist}{}{\setlength{\leftmargin}{0pt}%
\setlength{\rightmargin}{0pt}\setlength{\labelwidth}{0pt}%
\setlength{\labelsep}{0pt}\setlength{\itemindent}{0pt}}%
\item\noindent\textbf{Proof #1}}{\hfill\ensuremath{\blacksquare}\end{trivlist}}

% - Thomas macro ----------------

\newcommand{\ie}{\emph{i.e.}~}
\newcommand{\cf}{\emph{cf.}~}
\newcommand{\eg}{\emph{e.g.}~}
\newcommand{\al}{\emph{al.}~}
\newcommand{\espace}{\vspace*{1ex}}
\newcommand\eqdef{\mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny def}}}{=}}}

%% multiset braces
\newcommand*{\lmsbrace}{\lbrace\!\!\lbrace}
\newcommand*{\rmsbrace}{\rbrace\!\!\rbrace}

%% math hyphen character
\mathchardef\mhyphen="2D

\newcommand{\emparagraph}[1]{\espace\noindent\textbf{#1} ~}

\newcommand*{\Naturals}{{\normalfont\textsf{I\kern-.3ex N}}}
\newcommand*{\Reals}{{\normalfont\textsf{I\kern-.3ex R}}}
\newcommand{\C}{\ensuremath{\mathscr{C}}} 
%% End Macro Thomas
